Discreteness to Convexity: Promotion Planning via Simplotope Triangulation

Price promotion optimization is a computationally challenging problem central to supermarket operations, requiring simultaneous pricing decisions across multiple products and periods. This paper introduces a new formulation for price promotion by developing convex hull results for supermodular compositions of univariate functions over a simplotope. Leveraging this reformulation with Gurobi, we achieve substantial performance gains: instances with up to 125 products, 20 periods, and 5 price levels are solved in an average of 7 minutes, demonstrating the potential to handle even larger instances. Our exact solution methods extract 25--48\% additional profit from promotion planning relative to state-of-the-art heuristic approaches. Additionally, we extend the polynomially solvable cases from two to multiple price levels and expand our results to allow for multiplicative historical effects. Our core methodological innovation applies to a broad class of nonlinear discrete optimization problems. Specifically, our results convexify a class of nonlinear functions that includes monomials and the widely studied L natural function structure.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
